DBRAG: Multi-Table Retrieval-Augmented Generation for Complex Database Queries

Recent advancements in large language models have introduced new capabilities for reasoning over structured data, particularly through program-aided tools that can analyze tables. However, many existing methods address single-table scenarios or assume that the relevant tables are already provided. In practice, users often issue complex data exploration queries over entire databases, where relevant information may be distributed across multiple relations. In this work, we introduce DBRAG, a retrieval-augmented generation framework tailored for multi-table question answering. DBRAG first retrieves candidate tables using an offline table index, enriches their summaries with query-relevant rows, and uses an LLM to rerank the candidates. A program-aided reasoner then selects the required tables and executes operations over their full contents, keeping the initial prompt context compact. Experiments on the Spider, GeoQuery, and ATIS datasets used in this study demonstrate improvements in table retrieval and multi-table question answering.

==> figures/tex/varyparam.tex <==
  \begin{subfigure}[t]{0.48\linewidth}\centering
    \captionsetup{skip=3pt}
    % \begin{tikzpicture}
    %   \begin{axis}[
    %     ylabel={Recall@5},
    %     ylabel near ticks,
    %     line width=0.75pt,
    %     xtick={5, 20, 50},
    %     mark size=3pt,
    %     legend style={at={(1.3,1.1)}, anchor=south, font=\small, legend columns=2},
    %     every axis plot/.append style={thick},
    %     yticklabel style={font=\small},
    %     xticklabel style={font=\small},
    %     ylabel style={font=\small},
    %     xlabel style={font=\small},
    %     ymin=85,
    %     ymajorgrids=true,
    %     grid style=dashed,
    %     width=1.1\linewidth,
    %     height=1.1\linewidth
    %   ]
    %     \addplot [RandRow] [error bars/.cd, y dir=both, y explicit] coordinates {
    %       (5, 85.91) (10, 94.2) (20, 94.5) (50, 95.8)
    %     };
    %     \addlegendentry{Relevant Rows}
    %     \addplot [RelRow] [error bars/.cd, y dir=both, y explicit] coordinates {
    %       (5, 85.91) (10, 93.3) (20, 95.1) (50, 94.9)
    %     };
    %     \addlegendentry{Random Rows}
    %   \end{axis}
    % \end{tikzpicture}

    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            ylabel={Recall@5},
            ylabel near ticks,
            bar width=5pt,
            ymin=85, ymax=97,
            mark size=3pt,
            % ytick={92, 93, 94, 95, 96},
            legend style={at={(1.3,1.1)}, anchor=south, font=\small, legend columns=2},
            every axis plot/.append style={thick},
            yticklabel style = {font=\small},
            xticklabel style = {font=\small},
            ylabel style ={font=\small},
            xlabel style ={font=\small},
            symbolic x coords={5, 10, 20, 50},
            xtick=data,
            tick pos=left,
            % tick pos=left,
            width=1.1\linewidth,
            height=1.1\linewidth,
        ]
        % Plot commands
        \addplot[RandRow] coordinates {(5, 89.5) (10, 93.3) (20, 95.1) (50, 94.9)};
        \addplot[RelRow] coordinates {(5, 89.5) (10, 94.2) (20, 94.5) (50, 95.8)};
        \addlegendentry{Relevant Rows}
        \addlegendentry{Random Rows}
        % \legend{MT-RAG (random), MT-RAG}

        \end{axis}
    \end{tikzpicture}
    \centering
    \caption{Retrieved Tables (K)}
    \label{fig:varyk}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\linewidth}\centering
    \captionsetup{skip=3pt}
    \begin{tikzpicture}
      \begin{axis}[
        ylabel={Table EM(\%)},
        ylabel near ticks,
        xtick={1,10,20},
        line width=0.75pt,
        mark size=3pt,
        % Removed the invalid 'hide legend' key
        every axis plot/.append style={thick},
        yticklabel style={font=\small},
        xticklabel style={font=\small},
        ylabel style={font=\small},
        xlabel style={font=\small},
        ymajorgrids=true,
        grid style=dashed,
        width=1.1\linewidth,
        height=1.1\linewidth
      ]
        \addplot [RandRow] [error bars/.cd, y dir=both, y explicit] coordinates {
          (1, 44.8) 
          (2, 44.9) 
          (5, 46.0) 
          (10, 46.7)
          (20, 46.2)
        };
        \addplot [RelRow] [error bars/.cd, y dir=both, y explicit] coordinates {
          (1, 43.8) 
          (2, 44.4) 
          (5, 46.3) 
          (10, 46.3)
          (20, 45.1)
        };
      \end{axis}
    \end{tikzpicture}
    \centering
    \caption{Context Rows (L)}
    \label{fig:varyl}
  \end{subfigure}


